Thermal conduction in classical low-dimensional lattices

Deriving macroscopic phenomenological laws of irreversible thermodynamics from simple microscopic models is one of the tasks of non-equilibrium statistical mechanics. We consider stationary energy transport in crystals with reference to simple mathematical models consisting of coupled oscillators on a lattice. The role of lattice dimensionality on the breakdown of the Fourier's law is discussed and some universal quantitative aspects are emphasized: the divergence of the finite-size thermal conductivity is characterized by universal laws in one and two dimensions. Equilibrium and non-equilibrium molecular dynamics methods are presented along with a critical survey of previous numerical results. Analytical results for the non-equilibrium dynamics can be obtained in the harmonic chain where the role of disorder and localization can be also understood. The traditional kinetic approach, based on the Boltzmann-Peierls equation is also briefly sketched with reference to one-dimensional chains. Simple toy models can be defined in which the conductivity is finite. Anomalous transport in integrable nonlinear systems is briefly discussed. Finally, possible future research themes are outlined.

==> TEXT/lll.tex <==
While remaining in the realm of harmonic systems, we now consider the role
of disorder on transport properties. More specifically, we shall consider 
random-mass (or isotopically disordered) chains
\begin{equation}
  m_n \ddot q_n = q_{n+1} - 2q_n + q_{n-1} \quad . 
\label{eq:lin0}
\end{equation} 
Boundary conditions play a crucial role but will be for  the moment left
unspecified (see below). Before entering in a more detailed discussion it is
worth mentioning the general results by  Lebowitz and collaborators
\cite{CL71,OL74} that  rigorously showed that the system approach a unique
stationary nonequilibrium state for a large class of heat baths.

As it is known, the presence of disorder generally induces
localization of the normal modes of the chain and one may thus expect the
latter  to behave as perfect thermal insulator. Nonetheless, the actual 
situation turns out to be much more complicated depending on boundary
conditions and the properties of the thermostats. 


{\it Localization of the eigenmodes -}
To understand the transport properties it is first useful to recall some basic
facts about localization. For illustration, let us consider the example of a
disordered chain with two evenly-distributed types of particles. Some of the
numerically computed eigenvectors are shown in Fig.~\ref{f:eigen}. Upon
ordering them  with increasing eigenfrequencies, a distinct difference in their
localization properties can be recognized. Indeed, for small frequencies (upper
panel of Fig.~\ref{f:eigen}), randomness induces only a relatively weak
modulation of the amplitude; a partial localization can be recognized in the
intermediate panel, while a clear evidence of localization is visible only for
the high-frequency eigenvector  reported in the bottom panel.

\begin{figure}[tcb]  
\begin{center} 
\includegraphics*[width=7cm]{CHAP4/eigen.eps} 
\caption{The first, 41st and
100th eigenvector (from top to bottom) in a chain of 130 particles with random
masses with an even distribution of 1 and 1/2 values. The increasing
localization with increasing eigenvalue is transparent.} 
\label{f:eigen} 
\end{center}  
\end{figure} 

A rigorous investigation can be performed by
applying the transfer matrix approach to the eigenvalue equation. 
After inserting the expression $q_n = v_n e^{i\omega t}$ in Eq.~(\ref{eq:lin0}),
we obtain
\begin{equation}
\label{eq:stat}
    -m_n \omega^2 v_n = v_{n-1} - 2v_n + v_{n+1} .
\end{equation}
It is well known that the spectral properties of linear operators
involving the discrete Laplacian can be determined from a 
recursive equation for the new variable $R_n = v_n/v_{n-1}$.
The most known example where this approach has been 
successfully employed is that of Anderson quantum localization in the 
tight-binding approximation (see, e.g. \cite{DG84}. In the present context, 
Eq.~(\ref{eq:stat}) yields
\begin{equation}
    R_{n+1} = 2 - m_n \omega^2 - \frac{1}{R_n} ,
\label{eq:hyper}
\end{equation}
an equation that can be interpreted as a ``discrete time'' stochastic
equation. The mass $m_n$ plays the role of a noise source (with bias), 
whose strength is gauged by the frequency $\omega$. 
In particular, the inverse localization length $\gamma$ is given by
\begin{equation}
    \gamma = \langle \ln R_n \rangle ,
\label{eq:lyap}
\end{equation}
while the integrated density of states $I(\omega)$ follows from node counting
arguments, i.e. $I(\omega) = f$, where $f$ is the fraction of  negative $R_n$
values. In Fig.~\ref{f:local} it is shown that $I$ increases linearly for 
small $\omega$ and exhibits some irregular fluctuations at larger frequencies. 
The upper band edge (at $\omega \simeq 2.8$) is easily identifiable as the point above which
$I(\omega)$ remains constant and equal to 1. At 
variance with the standard Anderson problem where all eigenmodes
are exponentially localized, here $\gamma$ tends to zero for $\omega \to 0$.
This can be easily understood from equation 
(\ref{eq:hyper}): Since $\omega^2$ multiplies the stochastic term disorder
becomes less and less relevant in the  small frequency limit. In this limit,
one can thus resort to a perturbative approach. Let us start noticing that for 
$\omega= 0$, $R=1$ is a marginally stable  fixed point of the recursive equation
(\ref{eq:hyper}). For small $\omega$,  an intermittent process sets in: after a
slow drift driving $R_n$ below  1, a reinjection to values larger than 1 occours
and nonlinearity become suddenly relevant. The process repeats again
and again. By writing  $R_n = 1 + r_n$ and expanding in powers of $r_n$,
we find that the  dynamics in the vicinity of $R_n=1$ is described by 
\begin{equation}
    r_{n+1} = r_n - r_n^2 - \omega^2 \langle m \rangle + \omega^2 \delta m  
\label{eq:hypap}
\end{equation}
where we have included only the first nonlinear correction and written
separately the average value of the noise term. In the limit of small 
$\omega$, this equation can be approximated by the Langevin equation 
\begin{equation}
    \dot r = - r^2 - \omega^2 \langle m \rangle + \omega^2 \delta m  
\label{eq:hypapc}
\end{equation}
where the same notations we have kept for the sake of simplicity.
The corresponding Fokker-Planck equation writes
\begin{equation}
\frac{\partial P}{\partial t} = 
  \frac{\partial(r^2+ \omega^2 \langle m \rangle)P}{\partial r} + 
  \frac{\sigma_m^2}{2}
  \frac{\partial^2 P}{\partial r^2}
\label{eq:fokpla}
\end{equation}
where $\sigma_m^2=\langle m^2\rangle-\langle m\rangle^2$ stands for the 
variance of the mass distribution. Given the steady incoming and outcoming 
flow, the stationary solution can obtained by imposing 
\begin{equation}
  (r^2+ \omega^2 \langle m \rangle)P + \frac{\sigma_m^2}{2}
  \frac{dP}{dr} = C
\end{equation}
where $C$ represents the probability flux to be determined by imposing 
the normalization of the probability density $P$. Notice also that $C$ can
be identified with the integrated density of states $I(\omega)$, since it
corresponds to the probability that, at each iterate, $R_n$ is reinjected
to the right, i.e. the probability of having a node in the eigenvector.  
In the absence of disorder ($\sigma_m=0$), 
\begin{equation}
    I(\omega) = C = \frac{\sqrt{\langle m \rangle}}{\pi} \omega
\label{eq:intden}
\end{equation}
and, correspondingly,
\begin{equation}
  P_0(r) = \frac{1}{\pi} \frac{\omega \sqrt{\langle m \rangle}}
         {r^2+ \omega^2 \langle m \rangle}
\end{equation}
This approximation is already sufficient to reproduce the behaviour of
$I(\omega)$ at small frequencies, as in the limit of $\omega \to 0$ the
variance of the disorder goes to zero faster than the average value.
This is confirmed by comparing the dotted line in Fig.~\ref{f:local}
(corresponding to the analytic expression (\ref{eq:intden})) with the 
numerically determined integrated density.

\begin{figure}
\begin{center}
\includegraphics*[width=7cm]{CHAP4/local.eps}
\caption{Integrated density of states, $I(\omega)$ (solid line), and inverse 
localization length, $\gamma$ (dashed line), as a function of the frequency 
$\omega$ for a chain with mass disorder: the particles have either mass 1 or 
1/2 with equal probability. The dotted line corresponds to the analytic
expression (\ref{eq:intden}).  In the inset the inverse localization length 
is plotted in doubly logairthmic scales (circles) and compared
with the theoretical formula (\ref{eq:analoc}) - solid line.}
\label{f:local}
\end{center}
\end{figure}

On the other hand, the above approximation is not accurate enough to 
determine the localization length,
as disorder is totally disregarded. Indeed, the symmetry of $P_0$ implies
that $\gamma \approx \langle r \rangle = 0$. By going one step further, we
can write $P(r)$ as $P_0$ plus a small perturbation. A simple calculation 
shows that 
\begin{equation}
  P(r) =  P_0(r) + \frac{\omega^5 \sigma_m^2 r \sqrt{\langle m \rangle} }
         {\pi(r^2+ \omega^2 \langle m \rangle)^3}
\end{equation}
From expression (\ref{eq:lyap}) for the inverse localization
length $\gamma$, we find that 
\begin{equation}
  \gamma = \langle r \rangle = \frac{\omega^2 \sigma_m^2}{8 \langle m \rangle}
  ,\qquad {\rm for} \qquad \omega \longrightarrow 0
\label{eq:analoc}
\end{equation}
an equation derived in Ref.~\cite{MI70} (see Fig.~\ref{f:local}).

\begin{figure}
\begin{center}
\includegraphics*[width=7cm]{CHAP4/local2.eps}
\caption{Integrated density of states, $I(\omega)$ (solid line), and inverse 
localization length, $\gamma$ (dashed line) for a random-mass chain as in
Fig.~\ref{f:local} with the addition of a unit frequency on-site potential.} 
\label{f:local2}
\end{center}
\end{figure}

If we add an harmonic on-site potential to Eqs. (\ref{eq:lin0}), the 
corresponding scenario becomes analogous  to that of the 1d Anderson problem
with all eigenfunctions being exponentially localized. This is illustrated in
Fig.~\ref{f:local2} where we have added harmonic springs with unit constant
(i.e. a force term $-q_n$ acting on the $n$-th particle) to the chain with
random masses considered above. The lower band-edge is now strictly bounded
away from zero and the inverse localization length does not vanish.
 
{\it The temperature profile - }
In order to study the nonequilibrium properties, we need to include the 
coupling with the thermal reservoirs. Here below, we consider Langevin-type heat 
baths, as they allow an analytic treatment though limited to the weak-coupling 
regime.  The starting equation writes
\begin{equation}
  m_n \ddot q_n = q_{n+1} - 2q_n + q_{n-1} + \delta_{n1}(\xi_+ - \lambda 
  \dot q_1) + \delta_{nN}(\xi_- -\lambda \dot q_N)
\label{eq:lin1}
\end{equation} 
where for simplicity we have assumed $\lambda_+ = \lambda_-=\lambda$.
Although the equations are still linear, there is no general method
to derive an analytic solution for generic values of the coupling constant
$\lambda$. Accordingly, we restrict ourselves to considering the perturbative
regime  $\lambda \ll 1$. It is convenient to introduce the new variable
\begin{equation}
u_n = \sqrt{m_n} q_n \quad ,
\label{eq:change}
\end{equation}
which allows rewriting Eq.~(\ref{eq:lin1}) as
\begin{eqnarray}
  \ddot u_n = \frac{u_{n+1}}{\sqrt{m_n m_{n+1}}} - &2&\frac{u_n}{m_n} + 
              \frac{u_{n-1}}{\sqrt{m_n m_{n-1}}} + \nonumber \\ 
          & &  \frac{\delta_{n1}}{m_1}(\sqrt{m_1}\xi_+ -\lambda \dot u_1) + 
        \frac{\delta_{nN}}{m_N}(\sqrt{m_N}\xi_--\lambda \dot u_N) \ ,
\label{eq:lin2}
\end{eqnarray}
The advantage of this representation is that the operator describing
the bulk evolution is symmetric and, accordingly, is diagonalized by an 
orthogonal transformation. In other words, upon denoting with $e_n^k$ 
the $n$th component of the $k$th eigenvector, it turns out that 
$\sum_n e_n^k e_n^h = \delta_{kh}$ and $\sum_k e_n^k e_j^k = \delta_{nj}$. 

With reference to the new variables $U_k = \sum_n u_n e_n^k$, the equations 
of motion write as
\begin{equation}
 \ddot U_k = - \omega^2_k U_k - \lambda \sum_j C_{kj} \dot U_j + 
   \frac{e_1^k}{\sqrt{m_1}} \xi_+ + \frac{e_N^k}{\sqrt{m_N}} \xi_- 
\label{eq:newbase}
\end{equation}
where $-\omega^2_k$ is the real, negative $k$th eigenvalue of the unperturbed 
evolution operator and
\begin{equation}
  C_{kj} = \frac{e^k_1 e^j_1}{m_1} + \frac{e^k_N e^j_N}{m_N} \quad .
  \label{eq:matrix}
\end{equation}
Eqs. (\ref{eq:newbase}) show that the normal modes are coupled among 
themselves through the interaction with the reservoirs.
Standard stochastic calculus applied to the modal energy 
$E_k = (\dot U_k^2 + \omega_k^2U_k^2)/2$ shows that the stationarity
condition for the time average $\langle \dot E_k \rangle = 0$ implies 
\begin{equation}
 C_{kk} \langle \dot U_k^2 \rangle  + \sum_{j\ne k} C_{kj}
 \langle \dot U_k \dot U_j \rangle = T_+ \frac{(e_1^k)^2}{m_1}  +
    T_- \frac{(e_N^k)^2}{m_N}  .
\label{eq:tloc2}
\end{equation}
Let us now show that, in the small-coupling limit, this sum is negligible.
In fact, from the equality
\begin{equation}
\frac{d\langle \dot U_k U_h \rangle}{dt} = 0 ,
\end{equation}
we find that
\begin{equation}
\langle \dot U_k \dot U_h \rangle - \omega_k^2 \langle U_k U_h
 \rangle - \lambda \sum_j C_{jh} \langle \dot U_j U_h \rangle  = 0 
\end{equation}
By solving this equation together with the symmetric expression obtained by
exchanging $k$ and $h$, it is transparent that 
$\langle \dot U_k \dot U_h \rangle$ is proportional to $\lambda$  
for $k \ne h$. Accordingly, up to first order in $\lambda$, 
\begin{equation}
 \langle \dot U_k^2 \rangle = \frac{1}{C_{kk}} 
   \left(T_+ \frac{(e_1^k)^2}{m_1} + T_- \frac{(e_N^k)^2}{m_N} \right)  ,
\label{eq:tloc3}
\end{equation}
As a consequence, by neglecting first order corrections, the local 
temperature $T_n$ reads 
\begin{equation}
T_n  = \left\langle \left(\sum_k \dot U_k e_n^k \right)^2 \right\rangle 
  \approx 
\sum_{k=1}^{N} \frac{(e_n^k)^2}{C_{kk}} \left( T_+ \frac{(e_1^k)^2}{m_1} + 
  T_- \frac{(e_N^k)^2}{m_N} \right)
\label{eq:simpl2}
\end{equation}
This is basically the expression derived by Matsuda and Ishii \cite{MI70}. 
As a consistency check, one can easily verify that if
$T_+ =T_- =T$, the local temperature $T_n$ is equal to $T$ for all values of 
$n$ (this follows from the normalization condition on the eigenvectors).
Furthermore, the profile is flat also when $T_+ > T_-$ and the amplitude of all eigenvectors
is the same at the two chain-ends: in this case, $T_n=(T_+ + T_-)/2$. An 
obvious limiting case is the homogeneous chain. Generally speaking, even though
the dynamics of a generic disordered chain is statistically invariant under
left-right symmetry, the same does not hold true for each individual eigenvector.
This induces some spatial dependence that we  shall investigate in the
following. 

Visscher \cite{V71} challenged equation (\ref{eq:simpl2}) by arguing that
quasi-resonances could be generic enough to affect typical realizations of the
disorder. In fact, a crucial assumption in the  derivation of the expression
for the temperature profile is that cross-correlations in Eq.~(\ref{eq:simpl2})
are negligible. This is basically  correct unless pairs of frequencies are
sufficiently close to each other, in which case the resonance phenomena should
be properly taken into account. Visscher indeed discussed particular examples
of mass distributions, where a more refined theory is needed. However, as
long as one is interested in generic realizations, the problem is whether
quasi-degeneracies in the spectrum are sufficiently frequent to significantly
affect the overall validity of formula (\ref{eq:simpl2}). In all the cases 
we have considered this issue turned out to be practically irrelevant.

Formula (\ref{eq:simpl2}) does not allow to obtain an analytic form of
the profile since it requires the knowledge of the eigenvectors and, on the
other hand, the localization length alone  does not suffice to predict their
amplitude at the boundaries. Therefore numerical diagonalization of the 
Hamiltonian for each different realization of the disorder is required. 
In Fig.~\ref{f:profran}, we have plotted the stationary temperature profile 
for a single realization of the disorder versus the rescale lattice position
$x=n/N$. Strong fluctuations accompany an average decrease of the temperature 
from $T_+$ to $T_-$. 
 
\begin{figure} 
\begin{center} 
\includegraphics*[width=8cm]{CHAP4/profran.eps}
\caption{Temperature profile as predicted from Eq.~(\ref{eq:simpl2}) for 
a given realization of disorder in a chain of length $N=128$, with $T_+=10$
and $T_-=5$.}
\label{f:profran} 
\end{center} 
\end{figure} 

This suggests averaging over independent realizations of the disorder in order
to better investigate the convergence properties with the system size.
In Fig.~\ref{f:profluc}a we have plotted the profile averaged over 1000 
realizations. Upon increasing the chain length, the profile seems to slowly 
attain a linear shape, but sizeable deviations are still present for chains 
as long as $N=512$. Such a slow convergence is
confirmed in Fig.~\ref{f:profluc}b, where we plotted the sample-to-sample
variance $\sigma_T^2$ of the temperature field. Although its asymptotic
behavior is even less clear, it is at least evident that fluctuations do not
vanish in the thermodynamic limit. This is tantamount to saying that the
temperature profile is not a self-averaging quantity. 

\begin{figure} 
\begin{center} 
\includegraphics*[width=8cm]{CHAP4/profluc.eps}
\caption{(a) The disorder-averaged temperature profile as predicted from 
the formula (\ref{eq:simpl2}) for different chain lengths 
(dotted, dashed, dot-dashed and solid curves refer to $N=64$, 128, 256, 
and 512 respectively). (b) The variance of the temperature in the same 
notations as in panel (a).}
\label{f:profluc} 
\end{center} 
\end{figure} 


Such difficulties dramatically emerge when performing direct simulations of a
disordered chain. This issue is of great practical importance also in view of
more complex models where analytical results  are not available.  The major
problem is represented by the extremely slow convergence towards the asymptotic
regime that can be explained as follows. Eq.~(\ref{eq:newbase})  shows that
the effective coupling of each eigenmode with the reservoirs is proportional to
its square amplitude at the extrema. Therefore, all eigenmodes that are
localized away from the boundaries can thermalize only in astronomically long
times. To be more specific, the coupling strength of an  eigenmode
characterized by an inverse localization length $\gamma$ is of order
$\exp(-\gamma N)$, since it is localized a distance equal, on the average, to
the half of the chain length. This implies that the asymptotic profile is
attained over times that grow exponentially with $N$. In other words, the
stationary state is never reached in the thermodynamic limit. To practically
illustrate the issue, we have simulated a chain in contact with two stochastic
heat baths operating at the same temperature $T=5$ (see
Fig.~\ref{f:prof-flat}). To further emphasize the slow convergence, all atoms
have been  initially set at rest in their equilibrium positions. Even for
relatively short chains almost $10^6$ time units do not suffice to fully
thermalize the bulk.  A more direct way of looking at the convergence to the
flat temperature profile is by monitoring the cumulative time average $T_m$
performed on the 5 central sites (and averaged also over different realizations
of the disorder). The data reported in Fig.~\ref{f:temp-flat} with the choice
of a logarithmic scale for the time axis gives an idea of the time
needed to reach the equilibrium value $T_m = 5$.

\begin{figure} 
\begin{center}
\includegraphics*[width=7cm]{CHAP4/prof-flat.eps}
\caption{Average temperature profile of random-mass chains for $N=16$, 32 
and 64 (dotted, dashed and solid curve, respectively). The coupling constant is 
$\lambda = 1$. The average is performed over 1000 realizations of the disorder 
each of $5\cdot 10^5$ time units.}
\label{f:prof-flat} 
\end{center}
\end{figure} 



\begin{figure} 
\begin{center}
\includegraphics*[width=7cm]{CHAP4/temp-flat.eps}
\caption{Behaviour of the time average of the temperature in the 5 central
sites for $N=16$, 32 and 64 (dotted, dashed and solid curve, respectively).}
\end{center}
\label{f:temp-flat} 
\end{figure} 


{\it Heat flux - }
In the case of stochastic heats bath like those considered in the previous
section one can determine the total energy flux by using Eq.~(\ref{eq:flusto}).
By making use of Eq.~(\ref{eq:simpl2}) we obtain \cite{MI70,V71}
\begin{equation}
  J(\lambda,N) \; = \;\lambda (T_+-T_-)\sum_{k}
\frac{(e_1^k)^2(e_N^k)^2}{m_N(e_1^k)^2+m_1(e_N^k)^2} \; \equiv \;
 \sum_k J_k
\label{eq:fluxo}
\end{equation}
where the $k$th addendum $J_k$ is naturally interpreted as the contribution 
of the $k$th mode. As intuitively expected, the latter is 
larger for modes that have larger amplitudes at the boundaries and 
couple thus more strongly with the reservoirs. 
This interpretation can be justified from Eqs.~(\ref{eq:newbase}).
Indeed, in so far as cross-coupling can be neglected, the dynamics of the 
$k$th eigenmode is approximately described by the equation
\begin{equation}
 \ddot U_k = - \omega^2_k U_k - \lambda C_{kk} \dot U_k + 
   \frac{e_1^k}{\sqrt{m_1}} \xi_+ + \frac{e_N^k}{\sqrt{m_N}} \xi_-  .
\label{eq:newbase2}
\end{equation}
Standard stochastic calculus shows that, in the stationary regime, the 
energy exchanged per unit time with the two thermal baths is equal to $J_k$, 
where $J_k$ coincides with the expression implicitely defined by 
Eq.~(\ref{eq:fluxo}). 

However, heat transport is characterized by more subtle mechanisms than one 
could infer from this simple picture of independent modes. This is immediately 
understood if we look at the general expression for the local heat flux, 
Eq.~(\ref{eq:newflux}), that, in the case of harmonic chains, reduces to
\begin{equation}
\langle j_n \rangle = -\langle q_n \dot q_{n+1} \rangle .
\label{eq:nfluxhar}
\end{equation}
By expanding $q_n$ and $\dot q_{n+1}$ in eigenmodes, this equation 
can be rewritten as
\begin{equation}
\langle j_n \rangle = -\sum_{k,h=1}^N \frac{e^k_{n+1}e^{h}_{n}}
  {\sqrt{m_n m_{n+1}}} \langle U_k \dot U_h \rangle ,
\label{eq:nfluxex}
\end{equation}
an expression that, in spite of the explicit presence of the subscript $n$,
is independent of $n$. The interesting point that is made transparent by this
formula is that a nonvanishing flux is necessarily associated with the
existence of {\it correlations among different modes}. This is all the way 
more significative, once we realize that diagonal terms with $k=h$
vanish, being $\langle U_k \dot U_{k} \rangle$ the average of the 
derivative of a bounded function. This observation seems to be in contrast 
with the derivation of Matsuda-Ishii formula itself, that is basically obtained 
by treating all modes as evolving independently of each other. Anyway, we
should notice that the heat-flux is proportional to $\lambda$ and this is
compatible with the existence of weak modal correlations. In fact, 
``velocity-velocity'' or ``position-velocity'' correlations may arise from 
the fact that all eigenmodes are subject to the same noise source (except 
for a multiplicative factor) and this may well induce a sort of 
synchronization among them. 

The existence of this type of coherence has been numerically investigated 
and confirmed in Ref.~\cite{FMC98}, where the behaviour of a homogeneous 
harmonic chain has been thoroughly studied. Here below, we proceed with our 
perturbative analysis by deriving an analytic expression. Let us start by
noticing that the equality $d\langle U_k U_h \rangle/dt = 0$ implies that 
\begin{equation}
\langle \dot U_k U_h\rangle=- \langle \dot U_h U_k\rangle \, .
\end{equation}
This antisymmetry property together with the further equality 
$d\langle \dot U_k \dot U_h\rangle/{dt}=0$ imply that 
\begin{equation}
\lambda C_{kh} \left( \langle \dot U_k^2  \rangle +
     \langle \dot U_h^2 \rangle \right) - \left(\omega_k^2-\omega_h^2\right) 
  \langle \dot U_k U_h \rangle = 2 \lambda 
  \left( T_+\frac{e^k_1 e^h_1}{m_1} + T_-\frac{e^k_N e^h_N}{m_N} \right) 
\end{equation}
After replacing the expression of $\langle \dot U_k^2 \rangle$ (see 
Eq.~(\ref{eq:tloc3})) in the above equation, the latter can be solved for 
$\langle \dot U_k U_h\rangle$. 

Instead of discussing the general case, we prefer to illustrate the  presence
of these correlations in the simple case of a homogeneous harmonic chain (
see also Ref. \cite{FMC98}). In
this context, one can, in principle, obtain a a general expression for the
correlations by transforming  Eq.~(\ref{eq:zsol}) (derived for an arbitrary
$\lambda$ value) in $k$ space.  However, the calculations, though
straightforward, are rather tedious. Therefore, we limit ourselves to
considering the weak-coupling limit.  The symmetry of the eigenmodes imply
that  if $\delta = h-k$ is an even number correlations vanish, while for  an
odd $\delta$ we have 
\begin{equation}
  \langle \dot U_k U_{k+\delta} \rangle = 2 \frac{\lambda (T_+-T_-)}{m}
  \frac{e^k_1 e^{k+\delta}_1}{\omega_{k+\delta}^2-\omega_k^2} 
\label{eq:corana}
\end{equation}
In Fig.~\ref{f:cormod}a we report the numerical results for a chain of length 
$N=128$ with fixed boundary conditions and interacting with two thermal baths 
at temperatures $T_+ = 75$ and $T_-=25$.  Apart from the residual statistical
fluctuations, a reasonable agreement with expression (\ref{eq:corana}) is found
upon letting   $\lambda = 0.056$ (approximately equal to the inverse of the
average separation between consecutive collisions).   Fig.~\ref{f:cormod}b
shows  the results for the same length but a stronger  coupling strength. The
different shape of the curves is a clear indication that higher order terms
must be taken into account, since the perturbative approach implies that the
coupling constant acts just as a multiplicative factor. It is anyhow
interesting that shape itself is invariant under change of $\delta$ as it can
be seen in the inset where the three curves are rescaled to their maximum
value.

\begin{figure} 
\begin{center}
\includegraphics*[width=7cm]{CHAP4/cormod.eps}
\caption{
Modal correlations for a harmonic chain of length $N=128$ with fixed boundary
conditions.  Averaging has been performed on a time $t = 10^8$ units.  Solid,
dashed and dotted curves correspond to $\delta =1$, 3, and 5, respectively,
while the thin lines correspond to the analytic expressions (\ref{eq:corana}). 
(a) refers to a weak-coupling case: the times  between consecutive collisions
are  uniformly distributed in the interval $[19,21]$. (b) corresponds to a
strong coupling: collision times distributed in $[0.9,1.1]$.  The inset
cointains  the same curves, after rescaling to the maximum values. } 
\label{f:cormod} 
\end{center}
\end{figure} 

{\it The thermal conductivity - }
If obtaining an accurate analytic estimate of the flux is as difficult as
determining the temperature profile, we can at least make use of
Eq.~(\ref{eq:fluxo}) to determine its scaling properties. In fact, since
high-frequency eigenmodes are strongly localized, it is clear that only the
first part of the spectrum contributes significantly to the flux. Let thus
$N_e$ be the number of modes whose localization length is larger
than the sample size $N$. From  Eqs.~(\ref{eq:intden},\ref{eq:analoc}), it
follows that  $\gamma \simeq \sigma^2_m I(\omega)^2/\langle m \rangle$. Upon
writing $I = N_e/N$ and imposing $\gamma = 1/N$, we find that
\begin{equation} 
   N_e \; = \; \frac{\langle m \rangle}{\sigma_m}\sqrt{N} .
\end{equation} 
At this point, it becomes crucial to specify the boundary conditions.
Let us first consider the case of free ones: the square amplitude of
an extended eigenmode in a lattice of size $N$ is on the order $1/N$.
This implies that the contribution to the flux of one of such modes is
$\lambda (T_+-T_-)/N$ and the total flux can be estimated as 
\begin{equation} 
   J_{free}(\lambda,N) \; \propto \;
   \lambda (T_+-T_-) \frac{\langle m \rangle}{\sigma_m}
   \frac{1}{\sqrt{N}}.
\end{equation} 
As a result the conductivity diverges as 
\begin{equation} 
  \kappa_{free} \; \propto \;  
  \lambda \frac{\langle m \rangle}{\sigma_m}\sqrt{N} .
\end{equation} 
This scaling was first derived in Ref.~\cite{MI70} and later confirmed in
Ref.~\cite{KPW78} by means of a different approach. On the other hand, 
for fixed boundary conditions the result is completely different. In this 
case all eigenmodes must vanish for $n=0$ and $n=N+1$. By approximating the 
site-to-site variation of $e^k_n$ with the wavenumber $k/N$, we find that the 
square amplitude of $e^k_1$ and $e^k_N$ is on the order of $k^2/N^3$. As a
consequence, summing all such addenda up to $k=N_e$ yields (SIETE D'ACCORDO?)
\begin{equation} 
   J_{fix}(\lambda,N) \; \propto \;
   \lambda (T_+-T_-) \left(\frac{\langle m \rangle}{\sigma_m}\right)^3
   \frac{1}{{N}^{3/2}}.
\end{equation} 
and, accordingly, the thermal conductivity vanishes as  
\begin{equation} 
  \kappa_{fix} \; \propto \;  
  \lambda \left(\frac{\langle m \rangle}{\sigma_m}\right)^3
 \frac{1}{\sqrt{N}} .
\end{equation} 

The above estimates give only the leading orders in $N$. In view of
the previously encountered strong finite-size effects, it is   
crucial to check directly the convergence to the asymptotic results.
To this aim it is convenient to compute the effective exponent
\begin{equation}
\alpha_{ef}(N) \; = \;  \frac{d\ln \kappa}{d\ln N}
\label{logder}
\end{equation}
The results are shown in Fig.~\ref{f:der-flux} for the case of 
fixed boundaries. 
For weak coupling, the conductivity has been evaluated by numerically 
computing the eigenvectors and averaging of Matsuda-Ishii formula
(\ref{eq:fluxo}) over 1000 realizations of the disorder. The asymptotic regime
$\alpha = -1/2$ is approached very slowly (see the circles): one should
consider $N$ values much  greater than $10^3$. Similar results are found at
stronger coupling by directly simulating chains that interact with stochastic
baths. The  data (diamonds in Fig.~\ref{f:der-flux}) suggest that a relatively
strong  coupling reduces the amplitude of finite-size corrections. Finally, it
is important to  realize that the small coupling of the exponentially localized
modes with the termal baths does not cause any problem to the temporal
convergence of $J(\lambda,N)$, since independently of whether such modes have
reached  their stationary state, their contribution to the total flux is anyhow
negligible.

\begin{figure} 
\begin{center} 
\includegraphics*[width=7cm]{CHAP4/der-cond.eps}
\caption{The effective divergence exponent defined in (\ref{logder}) 
versus the chain length. The logarithmic derivative has been evaluated
with finite differences, subsequent points correspond to chain of 
double length. Circles are obtained from the Matsuda-Ishii formula, 
while diamonds correspond to a direct simulation of a chain interacting 
with stochastic baths operating at $T_+ = 10$ and $T_-=5$, respectively. 
The collision times were uniformely distributed 
in the range [1,2].}
\label{f:der-flux} 
\end{center} 
\end{figure} 

In summary, not only boundary conditions affect the scaling behaviour of
$\kappa$, but they give rise to qualitatively different scenarios: for free
boundaries, disordered harmonic chains exhibit an anomalous conductivity as it
diverges in the thermodynamic limit. On the contrary, a disordered chain with
fixed boundaries behaves as good insulator! This latter scenario is  brought to
an extremum if we add an on-site potential. In fact, we have already  mentioned
that all eigenfuctions become exponentially localized and this implies that
conductivity is exponentially small in $N$. This is again very much reminiscent
of the electrical conductivity of the Anderson problem [REFERENZA].

Dhar \cite{D01} went even further and showed how the scaling behaviour of the
conductivity with size depends also {\it on the spectral properties of the
heat baths}. More precisely, if $\kappa \propto N^\alpha$ then the  exponent
$\alpha$ is determined by the low-frequency behaviour of the noise spectrum.
This implies that a suitable choice of the  latter can even lead to a finite
conductivity! Such a scenario is less  unphysical than it may appear at a first
glance. Integrability of the motion implies that the only scattering mechanism
that determine the  heat resistance is the interaction with the baths. It is
therefore  reasonable that the actual way in which the latter transfer energy
among the  modes plays a crucial role. 

{\it Modal fluxes - } We conclude this section with a discussion of  the modal
fluxes $J_k$ as defined from Matsuda-Ishii formula (\ref{eq:fluxo}). Besides
providing a finer verification of the latter, the analysis is useful in
understanding the individual contributions of each ``channel'' to the
transport.  The spectra $J_k$ obtained for different chain lengths are reported
in  Fig.~\ref{f:flux-mais}. They have been scaled each to the maximum $J_M$,
while $k$  has been scaled to the wavenumber $k_M$ of the maximum itself. In
practice, this is asymptotically equivalent to scaling the vertical axis by a
factor $N^2$ and the horizontal axis by $1/\sqrt{N}$. We have preferred to
adopt this strategy in order to possibly get rid of the strong finite-size
corrections revealed by the previous analysis. Indeed, the good data collapse
(except for the right tail) noticeable in Fig.~\ref{f:flux-mais} is very
suggestive of the existence of an asymptotic spectrum. Additionally,  the
quadratic growth predicted for fixed b.c. is much more clear (set the inset)
than one could have expected from the scaling behaviour of the total flux for
the same chain lengths.

\begin{figure} 
\begin{center} 
\includegraphics*[width=7cm]{CHAP4/flux-mais.eps}
\caption{The flux (scaled to the maximum value) versus the wavenumber $k$
(scaled to the position of the maximum) for different chain-lengths (dotted,
dashed, dot-dashed and solid curves refer to $N=32$, 64, 128 and 256,
respectively. The same quanties are reported in doubly logarithmic scales 
in the inset, to show the quadratic growth for small $k$.}
\label{f:flux-mais} 
\end{center} 
\end{figure} 

Besides looking at the average heat fluxes $J_k$, we have studied their
sample-to-sample fluctuations, by computing the variance $\sigma_J^2$. The
relative variance plotted versus the scaled (as in the previous figure)
wavenumber indicate that fluctuations are independent of the chain length
(see the almost overlapping curves in Fig.~\ref{f:varflu}): this means that
$J_k$ is not a self-averaging quantity in the thermodynamic limit and this
holds true even for low $k$-wavenumbers whose behaviour results, in principle
from a spatial averaging over increasingly long spatial scales. More precisely,
we observe that the variance increases exponentially with $k$ starting
approximately from 0.26 for the longest wavelengths. Moreover, we have compared
the theoretical results with nonequilibrium simulations with stochastic heat
baths and collision times distributed uniformly in the interval [30,60]. The
data plotted in Fig.~\ref{f:conf}  reveal a very good agreement over various
orders of magnitude if the coupling constant is set equal to $1/54$.

\begin{figure} 
\begin{center} 
\includegraphics*[width=7cm]{CHAP4/varflu.eps}
\caption{The relative standard deviation versus the rescaled wavenumber
$k$ reveals a clear exponential growth.}
\label{f:varflu} 
\end{center} 
\end{figure} 

\begin{figure} 
\begin{center} 
\includegraphics*[width=7cm]{CHAP4/conf.eps}
\caption{Comparison between numerical results and the theoretical formula for
the heat flux (solid curve). The agreement is fairly good for both $N=32$ 
(squares) and $N=64$ (diamonds).}
\label{f:conf} 
\end{center} 
\end{figure} 



